Kimera-Multi: a System for Distributed Multi-Robot Metric-Semantic Simultaneous Localization and Mapping

We present the first fully distributed multi-robot system for dense metric-semantic Simultaneous Localization and Mapping (SLAM). Our system, dubbed Kimera-Multi, is implemented by a team of robots equipped with visual-inertial sensors, and builds a 3D mesh model of the environment in real-time, where each face of the mesh is annotated with a semantic label (e.g., building, road, objects). In Kimera-Multi, each robot builds a local trajectory estimate and a local mesh using Kimera. Then, when two robots are within communication range, they initiate a distributed place recognition and robust pose graph optimization protocol with a novel incremental maximum clique outlier rejection; the protocol allows the robots to improve their local trajectory estimates by leveraging inter-robot loop closures. Finally, each robot uses its improved trajectory estimate to correct the local mesh using mesh deformation techniques. We demonstrate Kimera-Multi in photo-realistic simulations and real data. Kimera-Multi (i) is able to build accurate 3D metric-semantic meshes, (ii) is robust to incorrect loop closures while requiring less computation than state-of-the-art distributed SLAM back-ends, and (iii) is efficient, both in terms of computation at each robot as well as communication bandwidth.

==> figures/diagram.tex <==
\begin{tikzpicture}[node distance = 40mm and 40mm, inner sep=5pt,thick,trim
		right=5cm,scale=0.5]
		%%%
		\tikzstyle{box}=[rectangle, very thick, draw, fill=#1, minimum
		width=12mm, minimum height=7mm, rounded corners=0.1cm]
		\tikzstyle{line} = [draw, -latex]
		\tikzstyle{dline} = [draw, latex-latex]
		%%%
		\node (images)        [box=white,align=center] {\footnotesize
		Stereo / Semantic / Depth Images};
		\node (imu)    		  [box=white,align=center,right= 1cm of images]
		{\footnotesize IMU};
		%\node (pointcloud)               [box=yellow!30,align=center,below= 1cm
		%of images,xshift=-2cm] {Convert to Point Cloud};
		%\node (denseStereoPointcloud)    [below= 1cm of pointcloud] {Dense Stereo Pointcloud};
		\node (semantics)                [box=blue!5,align=center,below= 0.5cm
		of images, xshift=-1cm] {\footnotesize Kimera Semantics};
		\node (incrementalMesh)          [below= 1cm of semantics,align=center]
		{\footnotesize Incremental\\\footnotesize Mesh};
		\node (pgmo)    	  			 [box=purple!40,align=center,below= 3.6cm of
		semantics] {\footnotesize Local Mesh Optimization};
		\node (vio)    	  [box=blue!4,align=center,below= 0.5cm of imu]
		{\footnotesize Kimera VIO};
		\node (bow)    	  [below= 0.4cm of vio,align=center] {\footnotesize BoW / 
		Descriptors / Keypoints};
		\node (lcd)    	  [box=orange!30,align=center,below= 0.35cm of bow,
		densely dashed, very thick] {\footnotesize Dist.\ Loop Closure Detection};
		\node (pcm)    	  [box=red!10,align=center,below= 0.35cm of lcd, densely
		dashed, very thick] {\footnotesize Dist.\ Outlier Rejection (PCM)};
		\node (dpgo)      [box=green!10,align=center,right= 2.31cm of pgmo,
		densely dashed, very thick] {\footnotesize Dist.\ PGO};
		\node (odometry)  [below= 0.45cm of vio, xshift=-3.1cm] {\footnotesize Odometry};
		\node (optimizedpg)  [left= 0.3cm of dpgo,align=center] {\footnotesize
		Optimized\\\footnotesize Pose Graph};
		%
		\node (optMesh)  [below= 0.7cm of pgmo,align=center] {\footnotesize
		Optimized Mesh};
		\node (optTraj)  [below= 0.7cm of dpgo,align=center] {\footnotesize Optimized Trajectory};
		%
		%\node (otherPcm)       [right= 1.5cm of pcm] {};
		%\node (otherDpgo)      [right= 1.5cm of dpgo] {};
		%\node (otherLcd)      [right= 1.5cm of lcd] {};
		%\node (other)      [above= 1.2cm of otherDpgo] {Other Robots};
		%
		%%%%%%%%%%%%%%%
		\path [line] (images) -- (semantics);
		\path [line] (images) -- (vio);
		%\path [line] (pointcloud) -- (denseStereoPointcloud);
		%\path [line] (denseStereoPointcloud) -- (semantics);
		\path [line] (semantics) -- (incrementalMesh);
		\path [line] (incrementalMesh) -- (pgmo);
		\path [line] (imu) -- (vio);
		\path [line] (vio) -- (odometry);
		\path [line] (vio) -- (bow);
		\path [line] (bow) -- (lcd);
		\path [line] (lcd) -- (pcm);
		\path [line] (pcm) -- (dpgo);
		\path [line] (odometry.south) |- (pcm);
		\path [line] (dpgo) -- (optimizedpg);
		\path [line] (optimizedpg) -- (pgmo);
		\path [line] (pgmo) -- (optMesh);
		\path [line] (dpgo) -- (optTraj);
%		\path [dline,dashed,thick] (dpgo) -- (otherDpgo);
%		\path [dline,dashed,thick] (pcm) -- (otherPcm);
%		\path [dline,dashed,thick] (lcd) -- (otherLcd);
		\draw [thick] ($(semantics.north west)+(-1.3,0.6)$)  rectangle
		($(dpgo.south east)+(2.5,-0.6)$);
		\draw [blue,very thick] ($(semantics.north west)+(-0.1,0.1)$)  rectangle	($(vio.south east)+(0.1,-0.1)$);
\end{tikzpicture}


